Cantonese Automatic Speech Recognition Using Transfer Learning from Mandarin

We propose a system to develop a basic automatic speech recognizer(ASR) for Cantonese, a low-resource language, through transfer learning of Mandarin, a high-resource language. We take a time-delayed neural network trained on Mandarin, and perform weight transfer of several layers to a newly initialized model for Cantonese. We experiment with the number of layers transferred, their learning rates, and pretraining i-vectors. Key findings are that this approach allows for quicker training time with less data. We find that for every epoch, log-probability is smaller for transfer learning models compared to a Cantonese-only model. The transfer learning models show slight improvement in CER.

==> backup.tex <==

% \begin{table}[t]
% \setlength{\tabcolsep}{4pt}
% \caption{ASR Performance}
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \textbf{Model} & \textbf{CER} & \textbf{Corr} & \textbf{Sub} & \textbf{Del} & \textbf{Ins} & \textbf{WER} \\ \hline
% LDA+MLLT & 60.3 & 48.2 & 21.1 & 9.7 & 8.5 & 67.1 \\ \hline
% TDNN & 47.5 & 57.6 & 32.2 & 10.1 & 5.1 & 53.2 \\ \hline
% No transfer*\tablefootnote{We were unable to decode this -- see Section \ref{ssec:error_sources}}. & N/A & N/A & N/A & N/A & N/A & N/A \\ \hline
% lr=0 & 129.6 & 16.8 & 73.5 & 9.7 & 46.4 & 153.4 \\ \hline
% lr=0.25 & 155.5 & 36.6 & 60.8 & 2.6 & 92.1 & 187.8 \\ \hline
% lr=1 & 178.0 & 32.3 & 66.2 & 1.5 & 110.2 & 205.3 \\ \hline
% \end{tabular}
% \label{table:1}
% \end{table}

% \begin{table}[t]
% \setlength{\tabcolsep}{4pt}
% \caption{ASR Performance, i-vector comparison}
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \textbf{Model} & \textbf{CER} & \textbf{Corr} & \textbf{Sub} & \textbf{Del} & \textbf{Ins} & \textbf{WER} \\ \hline
% BABEL & 155.5 & 36.6 & 60.8 & 2.6 & 92.1 & 187.8 \\ \hline
% AISHELL2 & 137.1 & 37.1 & 61.0 & 1.9 & 74.3 & 165.4 \\ \hline
% \end{tabular}
% \label{table:2}
% \end{table}

\section{Error Analysis}
\label{sec:errors}
Our transfer learning models had some issues that caused very poor performance. We have analyzed each part of the pipeline thoroughly, and have identified several factors that could contribute to this. We have done our best to address these concerns where possible, given our time and computational power constraints.

\subsection{Sample Rate and GMM Mismatch}
\label{ssec:sample_rate}
We suspect the main source of error is from the mismatch in sample rates of Cantonese and Mandarin -- 8 kHz and 16 kHz. Even though we upsampled everything to 16 kHz, the Cantonese data still lacks the full frequency range of the Mandarin data. This is especially problematic when i-vectors are involved, as it violates the assumptions of the GMM -- the means of each dataset are clustered completely differently. The downstream TDNN model uses the tied-triphone state alignments and i-vectors, and cannot relearn them adequately. Thus, there is a mismatch between the triphone alignments for the GMM and the objective the model is optimizing for. This is evident in the fact that CER is 60.1\% for just the LDA MLLT alignments, and over doubles after the TDNN training. In continued work, we will downsample both datasets to 8 kHz to use only frequencies that exist on both of them.

\subsection{Other Potential Error Sources}
\label{ssec:error_sources}
First, we have trained on only 25 hours of Cantonese. The best reported result from BABEL TDNN baseline model is 37.0\% CER, whereas our baseline model trained on 25 hours gives 47.5\% CER. A similar 30\% relative performance boost is expected using the full 215 hour dataset.


Our transfer learning model results above did not use cleaned alignments and triphones, whereas the BABEL model did. Thus we trained another transfer learning model with them. With lr=0.25, the CER after cleaning went up from 137.1\% to 170.0\%. This may be because cleaning significantly reduces the size of the training data -- after cleaning, only 31 iterations are performed, from 48 iterations originally.

Another thought we had was that we may have made mistakes in writing the Kaldi code for transfer learning. Indeed, our first models were missing 3 frames (2 vs. 5) layer connecting transferred layers to the new block, which caused much of the original network weights to not be used. We referred the given WSJ to RM script to fix this, but results barely improve (about 10\% absolutely). The reported results above use the latest model.

Finally, we hypothesize that the AISHELL2 recipe may just not work for the intricacies of the BABEL dataset. After all, the baseline model, a comparatively simple TDNN, is able to achieve well under 100\% CER. To further investigate if we were doing the transfer learning part wrong, we use the exact same network config file for AISHELL2 to create a new model for BABEL. No transfer learning is involved. The model trains fine, but for some reason, we cannot even decode the training data with it. We are using the same decoding method as with all the other models, and tried to debug it to no avail. This suggests that the alignments may be so off using this model architecture that decoding is all but impossible.

We have been relatively comprehensive about our debugging attempts and considerations. We have consulted the professor, as well as the official \texttt{kaldi-help} forum for help\footnote{\url{https://groups.google.com/d/msg/kaldi-help/49pvku1rxmw/thXqPGAbDQAJ}}\footnote{\url{https://groups.google.com/d/msg/kaldi-help/tBMHTFQcliQ/BhnQ_p2KAAAJ}}. Despite the poor results, we expect our findings of using lr=1.0 and using AISHELL2-trained i-vectors to be the best to hold after addressing the issues. We are optimistic that with a bit more effort, and a more straightforward TDNN model, that our transfer learning approach from Mandarin to Canotnese will show good results.


